Avalanche: A PyTorch Library for Deep Continual Learning

Continual learning is the problem of learning from a nonstationary stream of data, a fundamental issue for sustainable and efficient training of deep neural networks over time. Unfortunately, deep learning libraries only provide primitives for offline training, assuming that model's architecture and data are fixed. Avalanche is an open source library maintained by the ContinualAI non-profit organization that extends PyTorch by providing first-class support for dynamic architectures, streams of datasets, and incremental training and evaluation methods. Avalanche provides a large set of predefined benchmarks and training algorithms and it is easy to extend and modular while supporting a wide range of continual learning scenarios. Documentation is available at \url{https://avalanche.continualai.org}.

==> cover_letter.tex <==
The following submission is intended for the machine learning open source software section. 
Avalanche is an open source project released under the MIT license. The main website with the documentation, tutorials, and links to the source code is [1]. The software release to be reviewed is v0.3.1. 
Avalanche is an active project, with 56 contributors and 1.2k stars on github[2]. There are already a number of projects using Avalanche, including both research projects, challenges, and teaching-related activities ([3-6] are some examples).
A previous paper describing Avalanche was published in Jun 2021 in the proceedings of the CLVISION workshop at CVPR 2021 [7]. At that moment, Avalanche was at an early alpha stage. This new paper provides an updated overview of the library, its design, goals, and future directions. No part of [7] has been reused in this paper.

TODO: It is particularly appreciated if it includes suggestions of possible reviewers, explaining briefly why they are relevant to your work.

[1] https://avalanche.continualai.org/
[2] information from github statistics in Jan 2023
[3] Li, Duo, et al. "Technical report for iccv 2021 challenge sslad-track3b: Transformers are better continual learners." arXiv preprint arXiv:2201.04924 (2022).
[4] Lin, Zhiqiu, et al. "The CLEAR Benchmark: Continual LEArning on Real-World Imagery." Thirty-fifth Conference on Neural Information Processing Systems Datasets and Benchmarks Track (Round 2). 2021.
[5] New, Alexander, et al. "Lifelong learning metrics." arXiv preprint arXiv:2201.08278 (2022).
[6] Vincenzo Lomonaco, PhD course on Continual Learning at University of Pisa, ContinualAI and AIDA Doctoral Academy Course, https://course.continualai.org/
[7] Lomonaco, Vincenzo, et al. "Avalanche: an end-to-end library for continual learning." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021.

==> latex - Copia/cover_letter.tex <==
The following submission is intended for the machine learning open source software section. 
Avalanche is an open source project released under the MIT license. The main website with the documentation, tutorials, and links to the source code is [1]. The software release to be reviewed is v0.3.1. 
Avalanche is an active project, with 56 contributors and 1.2k stars on github[2]. There are already a number of projects using Avalanche, including both research projects, challenges, and teaching-related activities ([3-6] are some examples).
A previous paper describing Avalanche was published in Jun 2021 in the proceedings of the CLVISION workshop at CVPR 2021 [7]. At that moment, Avalanche was at an early alpha stage. This new paper provides an updated overview of the library, its design, goals, and future directions. No part of [7] has been reused in this paper.

TODO: It is particularly appreciated if it includes suggestions of possible reviewers, explaining briefly why they are relevant to your work.

[1] https://avalanche.continualai.org/
[2] information from github statistics in Jan 2023
[3] Li, Duo, et al. "Technical report for iccv 2021 challenge sslad-track3b: Transformers are better continual learners." arXiv preprint arXiv:2201.04924 (2022).
[4] Lin, Zhiqiu, et al. "The CLEAR Benchmark: Continual LEArning on Real-World Imagery." Thirty-fifth Conference on Neural Information Processing Systems Datasets and Benchmarks Track (Round 2). 2021.
[5] New, Alexander, et al. "Lifelong learning metrics." arXiv preprint arXiv:2201.08278 (2022).
[6] Vincenzo Lomonaco, PhD course on Continual Learning at University of Pisa, ContinualAI and AIDA Doctoral Academy Course, https://course.continualai.org/
[7] Lomonaco, Vincenzo, et al. "Avalanche: an end-to-end library for continual learning." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2021.
